3D Printing Meets Computational Astrophysics: Deciphering the Structure of Eta Carinae's Inner Colliding Winds

We present the first 3D prints of output from a supercomputer simulation of a complex astrophysical system, the colliding stellar winds in the massive (>120 M_Sun), highly eccentric (e ~ 0.9) binary star system Eta Carinae. We demonstrate the methodology used to incorporate 3D interactive figures into a PDF journal publication and the benefits of using 3D visualization and 3D printing as tools to analyze data from multidimensional numerical simulations. Using a consumer-grade 3D printer (MakerBot Replicator 2X), we successfully printed 3D smoothed particle hydrodynamics (SPH) simulations of Eta Carinae's inner (r ~ 110 au) wind-wind collision interface at multiple orbital phases. The 3D prints and visualizations reveal important, previously unknown 'finger-like' structures at orbital phases shortly after periastron (phi ~ 1.045) that protrude radially outward from the spiral wind-wind collision region. We speculate that these fingers are related to instabilities (e.g. thin-shell, Rayleigh-Taylor) that arise at the interface between the radiatively-cooled layer of dense post-shock primary-star wind and the fast (3000 km/s), adiabatic post-shock companion-star wind. The success of our work and easy identification of previously unrecognized physical features highlight the important role 3D printing and interactive graphics can play in the visualization and understanding of complex 3D time-dependent numerical simulations of astrophysical phenomena.

==> views_ApastronHighMdot.tex <==
VIEW={LOS}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
   PART={ApastronHighMdotPrimaryWind}
    VISIBLE=true
  END
    PART={ApastronHighMdotWWCR}
    VISIBLE=true
  END
END
VIEW={PrimaryWind}
 COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={ApastronHighMdotWWCR}
    VISIBLE=false
  END
END
VIEW={WWCR}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={ApastronHighMdotPrimaryWind}
    VISIBLE=false
  END
  PART={ApastronHighMdotBase}
    VISIBLE=false
  END
END


==> views_ApastronLowMdot.tex <==
VIEW={LOS}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
   PART={ApastronLowMdotPrimaryWind}
    VISIBLE=true
  END
    PART={ApastronLowMdotWWCR}
    VISIBLE=true
  END
END
VIEW={PrimaryWind}
 COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={ApastronLowMdotWWCR}
    VISIBLE=false
  END
END
VIEW={WWCR}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={ApastronLowMdotPrimaryWind}
    VISIBLE=false
  END
  PART={ApastronHighMdotBase}
   VISIBLE=false
  END
END


==> views_JoinedMesh.tex <==
VIEW={Initial}
  COO=-52.5 52.099998474121094 54.059993743896484
  C2C=-0.5105893015861511 0.8317983746528625 -0.21773844957351685
  ROO=229.600017353549
  ROLL=-30.18191267808559
  BGCOLOR=1.000000 1.000000 1.000000 
  LIGHTS=CAD
  RENDERMODE=Solid
END



==> views_JoinedMesh3.tex <==
VIEW={Initial}
  COO=66.62226867675781 62.471580505371094 54.082698822021484
  C2C=0.17930114269256592 -0.395890474319458 0.9006230235099792
  ROO=110.67704955026124
  ROLL=11.071547106841201
  AAC=60.000001669652114
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END


==> views_PeriastronHighMdot.tex <==
VIEW={LOS}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
   PART={PeriastronHighMdotPrimaryWind}
    VISIBLE=true
  END
    PART={PeriastronHighMdotWWCR}
    VISIBLE=true
  END
  PART={HighMdotBase}
    VISIBLE=true
  END
END
VIEW={PrimaryWind}
 COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={PeriastronHighMdotWWCR}
    VISIBLE=false
  END
END
VIEW={WWCR}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={PeriastronHighMdotPrimaryWind}
    VISIBLE=false
  END
  PART={PeriastronHighMdotBase}
    VISIBLE=false
  END
END


==> views_PeriastronLowMdot.tex <==
VIEW={LOS}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
   PART={PeriastronLowMdotPrimaryWind}
    VISIBLE=true
  END
    PART={PeriastronLowMdotWWCR}
    VISIBLE=true
  END
  PART={PeriastronLowMdotBase}
    VISIBLE=true
  END
END
VIEW={PrimaryWind}
 COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={PeriastronLowMdotWWCR}
    VISIBLE=false
  END
END
VIEW={WWCR}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={PeriastronLowMdotPrimaryWind}
    VISIBLE=false
  END
  PART={PeriastronLowMdotBase}
    VISIBLE=false
  END
END


==> views_Phase1p045HighMdot.tex <==
VIEW={LOS}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
   PART={Phase1p045HighMdotPrimaryWind}
    VISIBLE=true
  END
    PART={Phase1p045HighMdotWWCR}
    VISIBLE=true
  END
   PART={HighMdotBase}
    VISIBLE=true
  END
END
VIEW={PrimaryWind}
 COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={Phase1p045HighMdotWWCR}
    VISIBLE=false
  END
END
VIEW={WWCR}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={Phase1p045HighMdotPrimaryWind}
    VISIBLE=false
  END
  PART={Phase1p045HighMdotBase}
    VISIBLE=false
  END
END


==> views_Phase1p045LowMdot.tex <==
VIEW={LOS}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
   PART={Phase1p045LowMdotPrimaryWind}
    VISIBLE=true
  END
    PART={Phase1p045LowMdotWWCR}
    VISIBLE=true
  END
  PART={Phase1p045LowMdotBase}
    VISIBLE=true
  END
END
VIEW={PrimaryWind}
 COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={Phase1p045LowMdotWWCR}
    VISIBLE=false
  END
END
VIEW={WWCR}
  COO=-111.08837127685547 -124.99275207519531 120.93260955810547
  C2C=-0.316093772649765 0.2559675872325897 -0.9135454893112183
  ROO=510.620425316105
  ROLL=-4.500539283281516
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={Phase1p045LowMdotPrimaryWind}
    VISIBLE=false
  END
  PART={Phase1p045LowMdotBase}
    VISIBLE=false
  END
END

